Nested Diffusion Models Using Hierarchical Latent Priors

We introduce nested diffusion models, an efficient and powerful hierarchical generative framework that substantially enhances the generation quality of diffusion models, particularly for images of complex scenes. Our approach employs a series of diffusion models to progressively generate latent variables at different semantic levels. Each model in this series is conditioned on the output of the preceding higher-level models, culminating in image generation. Hierarchical latent variables guide the generation process along predefined semantic pathways, allowing our approach to capture intricate structural details while significantly improving image quality. To construct these latent variables, we leverage a pre-trained visual encoder, which learns strong semantic visual representations, and modulate its capacity via dimensionality reduction and noise injection. Across multiple datasets, our system demonstrates significant enhancements in image quality for both unconditional and class/text conditional generation. Moreover, our unconditional generation system substantially outperforms the baseline conditional system. These advancements incur minimal computational overhead as the more abstract levels of our hierarchy work with lower-dimensional representations.

==> figure/fig_noise_lvl.tex <==
\begin{figure}[t]
    \centering

    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/img_src/coco_baseline_0.png}
        \subcaption{$L = 1$}
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/img_src/coco_uncond_baseline_2.png}
        \subcaption{$L=2$}
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/img_src/coco_uncond_l3_0.png}
        \subcaption{$L=3$}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/img_src/coco_uncond_4_1.png}
        \subcaption{$L=4$}
    \end{subfigure}\hfill
    \hfill
    \caption{Unconditional image generation on the COCO dataset is performed across various hierarchical levels. At $L=1$, it corresponds to standard diffusion models. As more levels are stacked, the generated images exhibit more coherent visual structures and improved overall image quality.}
    %the model can almost perfectly reconstruct the input, indicating that $\hat{\vz}_1$ contains sufficient information about the image and $\mD_{\theta_0}$ functions more like a deterministic decoder than a generative model. As $\sigma_1$ increases, the information from $\hat{\vz}^1$ becomes more constrained, allowing $\mD_{\theta_0}$ to generate new, diverse images.}
    %RCG\citep{li2023self} proposes to use more compact representations, $\vz_1\in \mathbb{R}^{256}$, but we find it still almost perfect reconstruct the input despite the feature dimension is much smaller.}
\end{figure}

==> figure/fig_visual_sources.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=3cm]{example-image-a}
        \caption{Input Image}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=3cm]{example-image-a}
        \caption{Ours}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=3cm]{example-image-a}
        \caption{VAE}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=3cm]{example-image-a}
        \caption{RCG~\citep{li2023self}}
    \end{subfigure}
    \caption{Visual comparison for constructing latent variable using different visual representations. We demonstrate the genreated images using oracle ${\vz_2}$. For VAE, we apply spatial pooling to down sample the feature resolution to $\vz_2^{\rm{VAE}}\in \mathbb{R}^{8\times8\times4}$. RCG~\citep{li2023self} uses the final output of MoCo-V3,  $\vz_2^{\rm{RCG}}\in \mathbb{R}^{256}$. VAE doesn't learn semantic representation therefore $\vz_2^{\rm{VAE}}$ only preserve the color rather than coherent structure. Despite $\vz_2^{\rm{RCG}}\in \mathbb{R}^{256}$ adopts more compact representations, it could still almost perfectly reconstruct the input, highlighting the important to compress the conditional signal via $\sigma_2$.}
    \label{fig:compar_visual}
\end{figure}



==> figure/knn_figure_copy.tex <==
    
\begin{figure}[t]
\small
    \centering
\begin{minipage}{1.0\linewidth}
\begin{minipage}{0.11\linewidth}
    \centering
    {\small \textbf{Input Image}}
    \textcolor{black}{\rule[1ex]{\linewidth}{1pt}}
\end{minipage}\hfill
\begin{minipage}{0.44\linewidth}
    \centering
    {\small \textbf{Neighbored Images with CLIP Features}}
    \textcolor{black}{\rule[1ex]{\linewidth}{1pt}}
\end{minipage}\hfill
\begin{minipage}{0.44\linewidth}
    \centering
    {\small \textbf{Neighbored Images with VAE Features}}
    \textcolor{black}{\rule[1ex]{\linewidth}{1pt}}
\end{minipage}

\begin{minipage}{0.11\linewidth}
\vspace{0pt}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_0_0.png}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_0_1.png}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_0_2.png}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_0_3.png}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_0_4.png}
\end{minipage}\hfill

\begin{minipage}{0.11\linewidth}
\vspace{-12pt}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_1_0.png}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_1_1.png}
\centering
{1x1x256=256}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_1_2.png}
\centering
{4x4x64=1024}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_1_3.png}
\centering
{8x8x4=256}
\end{minipage}\hfill
\begin{minipage}{0.22\linewidth}
\includegraphics[width=1.0\textwidth]{figure/img_src/knn_img_folder/img_1_4.png}
\centering
{16x16x4=1024}
\end{minipage}\hfill
%\vspace{4pt} 
%\begin{tikzpicture}
%\hspace{10pt}
%$    \begin{scope}
%$      \draw[->, thick](2,5) -- (12,5) node[pos=0.5,below]{\scriptsize Decreasing feature dimensions and increasing semantic abstraction levels};
%$    \end{scope}
%\end{tikzpicture}
\end{minipage}
\caption{\textbf{Visualization of K-Nearest Neighbors (KNN) with different sources of latent features:} For each input image, neighboring images are displayed based on features extracted from different hierarchical levels, with their corresponding spatial dimensions (Height × Width × Channel) indicated below. This comparison spans two types of visual representations, each adjusted to maintain the same number of feature elements: CLIP representations, and VAE bottlenecks. Unlike the VAE, which focuses on low-level visual structures, CLIP emphasizes semantic representations, yielding more meaningful nearest neighbors. Our experiments demonstrate that running a diffusion model on latent space with well-structured neighbors is essential for enhancing generation quality.}
\label{fig:knn}
\end{figure}

==> figure/teaser_fig.tex <==
\twocolumn[{%
   \renewcommand\twocolumn[1][]{#1}%
   \vspace{-20pt}
   \maketitle%
   \begin{minipage}[t]{1.0\linewidth}%
    \centering
    \begin{figure}
        \centering
        \includegraphics[]{example-image-a}
        \caption{Caption}
        \label{fig:enter-label}
    \end{figure}
    \caption{Our proposed nested diffusion models generate images by employing a series of diffusion models to estimate hierarchical semantic representations. We illustrate this process using a 3-level hierarchical system, where images in each row are generated based on the representations of images outlined with red borders from the previous levels, along with image labels. As the hierarchy progresses, the similarity between generated images evolves from abstract semantic similarities to lower-level visual feature similarities.}
   \end{minipage}%
   \vspace{15pt}
}]%

==> iclr_table/ablate_table_old.tex <==
\begin{table}[t]
\small
\centering
\strutlongstacks{T}
\centering
\begin{tabular}{l|c|c|c|c}
Extra Feature Sources (Feature Shape)& L & shape of $\{\vz_l\}_{2=1}^L$ & $\{\sigma_l\}_{l=2}^L$ & FID$\downarrow$\\
\hline
None & 1 & - & - & 6.93\\
\hline
Final output of MoCo-V3 ($1\times1\times256$) & 2 & $\{1\times1\times256\}$&\{0.0\}&\\
\hline
Feature map of MoCo-V3 ($14\times14\times768$) & 2 & $\{6\times6\times56\}$&\{1.0, 0.0\}&\\
 & 2 & $\{6\times6\times64\}$&\{1.0, 0.0\}&\\
 & 3 & $\{8\times8\times64, 6\times6\times56\}$&\{1.0, 0.0\}&\\
\hline
VAE bottleneck ($32\times32\times4$) & 3 & $\{8\times8\times4, 6\times6\times4\}$&\{0.0, 0.0\}&\\
& 3 & $\{8\times8\times4, 6\times6\times 4\}$&\{1.0, 0.0\}&\\
\end{tabular}
\end{table}

==> iclr_table/in100_coco_cond.tex <==
\begin{table}[t]
\small
\centering
\strutlongstacks{T}
\centering
\begin{subtable}{\linewidth}
\centering\begin{tabular}{l|ccc|ccc}
& \multicolumn{3}{c}{w/o CFG} & \multicolumn{3}{c}{w/ CFG}\\
\hline
Model & $\sigma_{L}$ = 0.0 & 0.5 & 1.0 & $\sigma_{L}$ = 0.0 & 0.5 & 1.0\\
\hline
$L = 1$ & \textbf{24.73} & - & -  \\
$L = 2$ & 10.90 & \textbf{8.18} & 9.44  \\
$L = 3$ &  11.80 & 7.75 & \textbf{7.54}  \\ 
$L = 4$ & - & - & - \\
\hline
%\color{gray}{$L = 1$} & \multicolumn{3}{c|}{{\color{gray} text conditional generation}} & \color{gray}{6.30} & \color{gray}{-} & \color{gray}{-} & \color{gray}{-} \\
\end{tabular}
\caption{Unconditional image generation on COCO-2014}
\label{table:uncond_coco}
\end{subtable}

\begin{subtable}{\linewidth}
\centering\begin{tabular}{l|ccc|ccc}
& \multicolumn{3}{c}{w/o CFG} & \multicolumn{3}{c}{w/ CFG}\\
\hline
Model & $\sigma_{L}$ = 0.0 & 0.5 & 1.0 & $\sigma_{L}$ = 0.0 & 0.5 & 1.0\\
\hline
$L = 1$ & \textbf{14.98} & - & -  \\
$L = 2$ & 11.76 & \textbf{8.15} & 8.99  \\
$L = 3$ & 10.47 & \textbf{6.97} &  7.18  \\ 
\hline
\end{tabular}
\caption{Text-to-image generation on COCO-2014}
\label{table:uncond_coco}
\end{subtable}

\caption{
}
\label{table:uncond_in100_coco}
\end{table}

==> iclr_table/model_complexity.tex <==
\begin{table}
\footnotesize
\centering
\begin{tabular}{c|c|c|c|c|c|c}
     $L$ &  1 & 2 & 3 & 4 & $5$ & $1^*$\\
     \hline
     GFlops & 26.82 & 27.13 & 28.17 & 29.61 & 33.98 & 35.11 \\
     \hline
     Param(M) & 104 & 208 & 313 & 417 & 523 & 135\\
     \hline
     FID $\downarrow$ & 31.13 & 16.52 & 15.50 & 13.87 & \textbf{9.87} & 19.74 \\
\end{tabular}
\caption{\textbf{Comparison of multiple model configurations over model depth $L$.} Unlike baseline diffusion model ($L = 1^*$) whose computational complexity (GFlops) grows linearly with model parameters, our efficient hierarchical design only yields minimal GFlops growth with deeper models but achieves much better image quality than the baseline model with the same GFlops.}
\label{table:complexity}
\end{table}

==> table/ablation.tex <==
\begin{table}[!ht]
\small
\centering
\begin{minipage}[t]{0.25\linewidth}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcc}
Dataset &  Epochs & FID$\downarrow$\\
\hline
IN100  & 800 &\\
IN100 & 1600 &\\
COCO & 500&\\
COCO & 1000&\\
\end{tabular}
\caption*{(a) Image quality when training $N=5, \sigma=0.3$ model for longer epochs.}
}\end{minipage}%
\hfill%
\begin{minipage}[t]{0.3\linewidth}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
Models & $\sigma$ & FID\\
\hline
VAE & - & & \\
N = 1 (VAE latent) & - & & \\
N = 1 & - & 320M & \\
N = 2 & 0.3 & 320M & \\
N = 5 & 0.3 & 320M & \\
\end{tabular}
\caption*{(b)Image quality when we train diffusion model on VAE latent space.}
}\end{minipage}
\hfill%
\begin{minipage}[t]{0.35\linewidth}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}
Models & $\sigma$ & \# Params & GFlops & FID$\downarrow$\\
\hline
N = 1 & - & & \\
N = 1 & - & 320M & \\
N = 2 & 0.3 & 320M & \\
N = 5 & 0.3 & 320M & \\
\end{tabular}
\caption*{(c) Image quality on COCO dataset trained for 300 epochs when we try to scale add more parameters (N=1, 320M) to default diffusion model}
}\end{minipage}%

\caption{\xiao{TODO: Complete table and captions}. Benchmark image generation quality of proposed hierarchical diffusion model on ImageNet-100 dataset. $N$ indicates the total hierarchy levels}
\end{table}

==> table/coco.tex <==
\begin{table*}[t]
\small
\centering
\begin{minipage}[t]{1.0\linewidth}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccccc|lccccc}
Model & \# param & GFLOPS &$\sigma$ & FID$\downarrow$ & IS$\uparrow$&Model & \# param & GFLOPS &$\sigma$ & FID$\downarrow$ & IS$\uparrow$\\
\hline
N = 1 (Uncond) &59M & 28.83& - &&& N = 1(GT cond) &59M & 28.83& - &21.71&\\
%GT conditional & 59M & 28.83& - &21.71&\\
%N = 2 & 133M &28.98&0.0&&\\
N = 2 & 133M &28.98&0.3&&&N = 2 & 133M &28.98&0.0&&\\
N = 3 & 205M &29.31&0.3&16.49& & N = 5 & 320M &36.99&0.0&18.07&\\
N = 4 & 276M &30.87&0.3&&&N = 5 & 320M &36.99&0.1&13.05&\\
%N = 5 & 320M &36.99&0.0&18.07&\\
N = 5 & 320M &36.99&0.3&10.16&&N = 5 & 320M &36.99&0.2&10.75&\\
\end{tabular}
\caption{\xiao{TODO: Complete table and captions}. Benchmark image generation quality of proposed hierarchical diffusion model on ImageNet-100 dataset. $N$ indicates the total hierarchy levels}
}\end{minipage}
\end{table*}

==> table/coco_split.tex <==
\begin{table*}[t]
\small
\centering
\begin{minipage}[t]{0.6\linewidth}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccc}
Model  & Train FID$\downarrow$ & Val FID $\downarrow$\\
\hline
EDM~\citep{karras2022elucidating}& 26.93 &33.79&\\
RCG~\citep{li2023self}&21.61&28.32&\\
Ours (L = 5,$\sigma$ = 0.2)&\textbf{10.46}&\textbf{17.09}&\\
\hline
Ours (L = 5,$\sigma$ = 0.2, 1000 epochs)&8.34&13.95&\\
\end{tabular}
\captionof{table}{(a) caption for hierarchical model}
\label{tab:coco_exp}
}\end{minipage}%
\hfill%
\begin{minipage}[t]{0.35\linewidth}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccc}
$\sigma$ & Train FID$\downarrow$ & Val FID $\downarrow$\\
\hline
0.0&14.38&20.97&\\
0.1&11.91&18.49&\\
0.2&\textbf{10.46}&\textbf{17.09}&\\
0.3&11.09&17.73&\\
\end{tabular}
\captionof{table}{(a) caption for hierarchical model}
\label{tab:coco_ablate_sigma}
}\end{minipage}
\end{table*}

==> table/imagenet_100.tex <==
\begin{table*}[t]
\small
\centering
\begin{minipage}[t]{1.0\linewidth}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccccc|lccccc}
Model & \# param & GFLOPS &$\sigma$ & FID$\downarrow$ & IS$\uparrow$&Model & \# param & GFLOPS &$\sigma$ & FID$\downarrow$ & IS$\uparrow$\\
\hline
N = 1 (Uncond) &59M & 28.83& - &&& N = 1(GT cond) &59M & 28.83& - &21.71&\\
%GT conditional & 59M & 28.83& - &21.71&\\
%N = 2 & 133M &28.98&0.0&&\\
N = 2 & 133M &28.98&0.3&&&N = 2 & 133M &28.98&0.0&&\\
N = 3 & 205M &29.31&0.3&16.49& & N = 5 & 320M &36.99&0.0&18.07&\\
N = 4 & 276M &30.87&0.3&&&N = 5 & 320M &36.99&0.1&13.05&\\
%N = 5 & 320M &36.99&0.0&18.07&\\
N = 5 & 320M &36.99&0.3&10.16&&N = 5 & 320M &36.99&0.2&10.75&\\
\end{tabular}
\caption{\xiao{TODO: Complete table and captions}. Benchmark image generation quality of proposed hierarchical diffusion model on ImageNet-100 dataset. $N$ indicates the total hierarchy levels}
}\end{minipage}
\end{table*}

==> table/imagenet_100_split.tex <==
\begin{minipage}[t]{1.0\linewidth}{
\begin{minipage}[b]{0.5\linewidth}{
\centering
\label{tab:ablate lvl imagenet}
\setlength{\tabcolsep}{3.5pt}
\captionsetup{type=table}
\begin{tabular}{lcccccc}
Model & \# param & GFLOPS & Train FID$\downarrow$ & Val FID$\downarrow$ & IS$\uparrow$\\
\hline
L = 1  &59M & 28.83& - &&\\
%GT conditional & 59M & 28.83& - &21.71&\\
%N = 2 & 133M &28.98&0.0&&\\
L = 2 & 133M &28.98&&\\
L = 3 & 205M &29.31& 16.49&20.92&22.09 \\
L = 4 & 276M &30.87& 13.33&18.12&24.16\\
%N = 5 & 320M &36.99&0.0&18.07&\\
L = 5 & 320M &36.99& 10.16&15.57&26.25\\
\end{tabular}
\captionof{table}{Ablation of total hierarchy}
}\end{minipage}%
\hfill
\begin{minipage}[b]{0.25\linewidth}{
\captionsetup{type=figure}
\includegraphics[width=1.0\textwidth]{example-image-a}
\captionof{table}{Ablation for sigma over training}
\label{fig :sigma imagenet}
}\end{minipage}
}\end{minipage}

==> table/main_table_coco.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lccccc}
\centering
Model & Condition Signal & \#Param & GFLOPs & Train FID$\downarrow$ & Val FID $\downarrow$\\
\hline
EDM~\citep{karras2022elucidating} & No &59M & 28.83& &\\
RCG~\citep{li2023self} & Self-generated & 133M &28.98&0.3&16.49\\
Ours (N = 2,$\sigma$ = 0.3) & Self-generated & 133M &28.98&0.3&16.49\\
Ours (N = 5,$\sigma$ = 0.3) & Self-generated & 320M &36.99&0.3&16.49 \\
Ours (N = 5,$\sigma$ = 0.3)(1000 epochs) & Self-generated & 320M &36.99&0.3&16.49 \\
\end{tabular}
\caption{\xiao{TODO: Complete table and captions}. Benchmark image generation quality of proposed hierarchical diffusion model on COCO dataset.}
\label{tab:main_table_coco}
\end{table*}

==> table/main_table_imagenet100.tex <==
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc|ccc}
\centering
Model & Condition& \#Param / M & GFLOPs &  Train FID$\downarrow$ & Val FID $\downarrow$& IS$\uparrow$\\
\hline
EDM~\citep{karras2022elucidating} & No &59 & 28.83& & &\\
EDM~\citep{karras2022elucidating} & GT Label &59 & 28.83& & & \\
VAE + DiT~\citep{peebles2023scalable} & No & 72 + 136 &59.31 + 11.88& 0.3&&\\
RCG ~\citep{li2023self} & Self-gen& 133 &28.98&0.3&16.49& \\
Ours (L = 5,$\sigma$ = 0.3) & Self-gen& 320 &36.99&0.3&16.49& \\
\end{tabular}
\caption{\xiao{TODO: Complete table and captions}. Benchmark image generation quality of proposed hierarchical diffusion model on ImageNet-100 dataset. \becca{RCG is performing EXACTLY the same as our method? } \xiao{Most numbers in this tables are place holders and we're filling the results now. Sorry for the confusion.}}
\label{tab:main_table_imagenet_100}
\end{table*}
